Hypothesize and Bound: A Computational Focus of Attention Mechanism for Simultaneous 3D Shape Reconstruction, Pose Estimation and Classification from a Single 2D Image

This article presents a mathematical framework to simultaneously tackle the problems of 3D reconstruction, pose estimation and object classification, from a single 2D image. In sharp contrast with state of the art methods that rely primarily on 2D information and solve each of these three problems separately or iteratively, we propose a mathematical framework that incorporates prior "knowledge" about the 3D shapes of different object classes and solves these problems jointly and simultaneously, using a hypothesize-and-bound (H&B) algorithm. In the proposed H&B algorithm one hypothesis is defined for each possible pair [object class, object pose], and the algorithm selects the hypothesis H that maximizes a function L(H) encoding how well each hypothesis "explains" the input image. To find this maximum efficiently, the function L(H) is not evaluated exactly for each hypothesis H, but rather upper and lower bounds for it are computed at a much lower cost. In order to obtain bounds for L(H) that are tight yet inexpensive to compute, we extend the theory of shapes described in [14] to handle projections of shapes. This extension allows us to define a probabilistic relationship between the prior knowledge given in 3D and the 2D input image. This relationship is derived from first principles and is proven to be the only relationship having the properties that we intuitively expect from a "projection." In addition to the efficiency and optimality characteristics of H&B algorithms, the proposed framework has the desirable property of integrating information in the 2D image with information in the 3D prior to estimate the optimal reconstruction. While this article focuses primarily on the problem mentioned above, we believe that the theory presented herein has multiple other potential applications.

==> LetterEditor.tex <==
The graphical model defined in this section is similar to the graphical model used in \cite{RotICCV09} but with two major differences. The first difference is that the unknown shapes $q$ and $v$ in this model are continuous, while in the model in \cite{RotICCV09} they are discrete; this allows us to compute tighter bounds for the evidence $L(H)$ (defined in \eqref{eq:Evidence} in Section \ref{sec:EvidenceDefinition}). The second difference is that in the current model the bias in the projection term $\log{P(q|v)}$ in \eqref{eq:LogProbability1} has been corrected (this is explained in detail in the next section). The graphical model defined in this section is also very similar to the graphical model introduced in \cite{Rot10}. The main difference in this case is that both the shape prior $B_K$ (in level 2 of Fig. \ref{fig:FactorGraph}) and the desired reconstruction $v$ (in level 3) are 3D entities, while the BF $B_f$ corresponding to the input image is two dimensional. In contrast in \cite{Rot10} the BFs corresponding to both the shape prior $B_H$ and the input image $B_f$ are 2D.


==> Proofs.tex <==
\section{Supplementary material: Proofs}
\label{sec:Proofs}

This section contains the proofs of the theorems that were only stated in the main text.

% Proposition 1.
\setcounter{proposition}{\ref{prop:FormProjectionFunction}}
\addtocounter{proposition}{-1}
\begin{proposition}[Form of the projection function]
Let us denote by $1_{(u,w)}$ a shape in a ray that consists on the interval $(u,w)$, and let $g$ be an independent and scale invariant projection function that satisfies the condition
\begin{equation}
g(1_{(1,e)}) = e^{\alpha}, \qquad \text{for some} \ \alpha < 0. 
\tag{\ref{eq:BorderCondition}}
\end{equation}
Let $v$ be a 3D continuous shape, and let 
\begin{equation}
\ell_v(\vec{x}) \triangleq \int_0^{\infty}{\frac{v_{R(\vec{x})}(r)}{r} \ dr} = \int_0^{\infty}{\frac{v(\vec{c}+r\vec{x})}{r} \ dr}
\tag{\ref{eq:DefLx}}
\end{equation}
be a measure of the ``mass" in the ray $R(\vec{x})$. Then the projection function $g$ must have the form
\begin{equation}
\tag{\ref{eq:FormProjectionFunction}}
g \left(v_{R(\vec{x})}\right) = e^{\alpha \ell_v(\vec{x})}.
\end{equation}
\begin{proof}
\hspace{-4pt}: To prove this theorem we proceed in two steps. First we find the functional form of the projection function for the particular family of shapes in a ray that consists of a single open interval, \ie $v_{R(\vec{x})} = 1_{(u,w)}$. Second, having a functional form for this family of 1D shapes, we extend the functional to shapes that can be written as the disjoint union of members of this family. This proves the proposition because any shape in a ray, being an open set in the ray, can be written in that form \cite[Proposition 2.9]{Kah95}.

More formally, we will prove the following two statements (for convenience we will write $g(u,w)$ instead of $g\left(1_{(u,w)}\right)$):

1) Consider an interval of the form $(u, w)$, where $u,w \in \mathbb{R}$ and $0 < u < w$. Then 
\begin{equation}
g(u,w) = \left(\frac{w}{u} \right)^\alpha.
\label{eq:PF1}
\end{equation}

2) Consider the shape $v_{R(\vec{x})}$ in ray $R(\vec{x})$, defined by
\begin{equation}
v_{R(\vec{x})} = \bigcup_i{(u_i, w_i)},
\label{eq:PF2}
\end{equation}
where the intervals are defined as in 1) above, and are disjoint. Then \eqref{eq:FormProjectionFunction} holds, with $\ell_v(\vec{x})$ defined as in \eqref{eq:DefLx}.

\paragraph{Proof of 1).}
Let us choose $p_L, q_L \in \mathbb{N}$, such that $e^{p_L / q_L} $ $\le w /u$ and let us also define $\beta \triangleq e^{1/q_L}$. Then from \eqref{eq:BorderCondition} and the independence and scale invariance of $g$, it follows that 
\begin{align}
e^{\alpha} = g(1, e) = g(1, \beta^{q_L}) & = \prod_{i=0}^{q_L-1}{g(\beta^i, \beta^{i+1})} = {g(1,\beta)}^{q_L} .
\label{eq:PF11}
\end{align}
Similarly,
\begin{align}
g\left(u, u e^{p_L / q_L}\right) & = g\left(1, e^{p_L / q_L}\right) = g\left(1, \beta^{p_L}\right) = {g(1,\beta)}^{p_L}.
\label{eq:PF12}
\end{align}
Therefore, substituting $g(1,\beta)$ from \eqref{eq:PF11} into \eqref{eq:PF12}, we obtain
\begin{equation}
g\left(u, u e^{p_L / q_L}\right) = e^{\alpha p_L / q_L}.
\end{equation}
Now, since $\left(u, u e^{p_L / q_L}\right) \subseteq (u, w)$ it follows from the monotonicity of $g$ that $g(u, w) \le g\left(u, u e^{p_L / q_L}\right)$.

Analogously, defining $p_U, q_U \in \mathbb{N}$ such that $e^{p_U / q_U} \ge w /u$ we prove that $g(u,w) \ge g(u,u e^{p_U/q_U})$. Therefore, making $e^{p_L / q_L} \to {(w / u)}^-$ and $e^{p_U / q_U} \to {(w / u)}^+$, we prove \eqref{eq:PF1}. \qed

\paragraph{Proof of 2).}
Since the intervals on the rhs of \eqref{eq:PF2} are disjoint, from the independence of $g$ and from \eqref{eq:PF1}, it follows that
\begin{equation}
\log{g \left(v_{R(\vec{x})}\right)} = \sum_{i}{\log{g(u_i, w_i)}} = \alpha \sum_{i}{\log{\frac{w_i}{u_i}}}.
\end{equation}
Defining $\ell(\vec{x})$ as in \eqref{eq:DefLx}, this expression is equal to 
\begin{align}
\log{g \left(v_{R(\vec{x})}\right)} & = \alpha \sum_{i}{\int_{u_i}^{w_i}{\frac{dr}{r}}} = \alpha \int_0^{\infty}{\frac{v_{R(\vec{x})}(r) }{r} \ dr} \nonumber \\
& = \alpha \ell_v(\vec{x}),
\end{align}
proving the theorem.\qed
\end{proof}
\end{proposition}

% Proposition 2.
\begin{proposition}[Explicit form of $u_{\Phi}(T)$]
\label{prop:RatioUnitSizes}
Let $T_c$ be a central dilation whose center is at the camera center $\vec{c}$ (\ie, $T_c(\vec{X}) \triangleq S(\vec{X} - \vec{c}) + \vec{c}$, $S>0$). Let $S_1 \triangleq (q_1,v_1,K,T_1)$ and $S_2 \triangleq (q_2,v_2,K,T_2)$ be two tentative solutions to our problem related by $T_c$ (\ie, $T_2 = T_c \circ T_1$ and $v_2(\vec{X}) = v_1({T_c}^{-1}(\vec{X}))$) that produce the same projection in the image sphere (\ie, $q_1 = q_2 = q$ and $P\left(q(\vec{x}) | v_{1, R(\vec{x})} \right) = P\left(q(\vec{x}) | v_{2,R(\vec{x})} \right) \ \forall \vec{x} \in \Theta$).

If the equivalent unit size $u_{\Phi}$ has the form $u_{\Phi}(T_i) = |J(T_i)|/\lambda'$, where $|J(T_i)|$ is the Jacobian of the transformation $T_i$, and $\lambda' > 0$ is an arbitrary constant, then we have $P(f,q_1,v_1,K,T_1) = P(f,q_2,v_2,$ $K,T_2)$ (as defined in \eqref{eq:JointProbability}).

In other words, this theorem states that if the equivalent unit size is chosen in the particular form defined above, 3D reconstructions related by a similarity transformation ($T_c$) that produce the exact same projection on the image sphere are equally preferred by the framework.
\begin{proof}
\hspace{-4pt}: To prove this proposition note that the first, second and fourth terms on the rhs of \eqref{eq:JointProbability} are equal for both solutions. The first terms are equal because $q_1 = q_2$ by hypothesis, and $f$ is common for all solutions. The second terms are equal because, by hypothesis, $v_1$ and $v_2$ produce the same projection on the image sphere. And the fourth terms are also equal because we assume that all hypotheses are, \emph{a priori}, equally likelly. Therefore we need to choose $u_{\Phi}$ to get the shape prior terms to be equal, \ie, we need $P(v_1|K,T_1) = P(v_2|K,T_2)$ (these quantities are defined in \eqref{eq:ShapePriorTerm}).

Defining $u_{\Phi}(T_2)$ as above, the third term for $S_2$, $\log{P(v_2|K,T_2)}$, is equal to
\begin{equation}
\frac{\lambda'}{|J(T_2)|} \int_{\mathbb{R}^3}{\log{P\Big(B_{K,T_2}(\vec{X}) = v_2(\vec{X})\Big)} \ d\vec{X}}.
\label{eq:TermPrior2}
\end{equation}
Now, since
\begin{align}
B_{K,T_2}(\vec{X}) & = B_K({T_2}^{-1}(\vec{X})) = B_K({T_1}^{-1} \circ {T_c}^{-1}(\vec{X})) \nonumber \\
& = B_{K, T_1}({T_c}^{-1}(\vec{X})),
\end{align}
\eqref{eq:TermPrior2} is equal to 
\begin{equation}
\frac{\lambda'}{|J(T_2)|} \! \int_{\mathbb{R}^3}{\! \log{P\Big(B_{K,T_1} ({T_c}^{-1}(\vec{X})) \! = \! v_1({T_c}^{-1}(\vec{X}))\Big)} \ d\vec{X}}.
\label{eq:TermPrior3}
\end{equation}
Making the change of variables $\vec{Y} = {T_c}^{-1}\vec{X}$, this expression is transformed into
\begin{equation}
\frac{\lambda' |J(T_c)|}{|J(T_2)|} \int_{\mathbb{R}^3}{\log{P(B_{K,T_1}(\vec{Y}) = v_1(\vec{Y}))} \ d\vec{Y}}.
\label{eq:TermPrior4}
\end{equation}

On the other hand the third term for $S_1$, $\log{P(v_1|K,}$ $T_1)$, is equal to 
\begin{equation}
\frac{\lambda'}{|J(T_1)|} \int_{\mathbb{R}^3}{\log{P (B_{K,T_1}(\vec{Y}) = v_1(\vec{Y}))} \ d\vec{X}},
\label{eq:TermPrior5}
\end{equation}
which is equal to \eqref{eq:TermPrior4} because $|J(T_2)| = |J(T_c)| |J(T_1)|$, proving the theorem. \qed
\end{proof}
\end{proposition}

% Lemma: Bounding the Projection Term.
\setcounter{lemma}{\ref{lem:UBProjectionTerm}}
\addtocounter{lemma}{-1}
\begin{lemma}[Upper bound for the projection term]
Let $\left(\Pi(\Theta), \Pi(\Phi)\right)$ be a standard partition and let $\tilde{q}$ and $\tilde{v}$ be two semidiscrete shapes in $\Pi(\Theta)$ and $\Pi(\Phi)$, respectively. Let $q$ and $v$ be two continuous shapes in $\Theta$ and $\Phi$, respectively, and define  
\begin{equation}
\Lambda_{\Theta}(q,v) \triangleq \int_{\Theta}{\log{P\left(q(\vec{x})|\ell_v(\vec{x})\right)}\ d\vec{x}},
\tag{\ref{eq:DefBigLambda}}
\end{equation}
with the integrand of this expression defined as in \eqref{eq:ProjectionTermForm}. Then:

1. Any continuous shape $q_*$ such that $q_* \sim \tilde{q}$ and the continuous shape $v_*$ defined by 
\begin{align}
v_*(\vec{X}) \!= \!\left\{\begin{array}{cc}
\!\!1 & \text{if } \vec{X} \! \in \bigcup_{j,i}{\Big[\Theta_j^1 \! \times \! [r_{i-1}, \rho_{j,i}^1] \cup \Theta_j^0 \!\times \! [\rho_{j,i}^0, r_i] \Big]} \\
\!\!0 & \text{otherwise},
\end{array} \right.
\tag{\ref{eq:VStar}}
\end{align}
(Fig. \ref{fig:BoundProjection}), where the quantities $\Theta_j^0$, $\Theta_j^1$, $r_i$, $\rho^1_{j,i}$ and $\rho^0_{j,i}$ are defined in \eqref{eq:Theta0}-\eqref{eq:Theta1}, \eqref{eq:r_i}, \eqref{eq:Rho1} and \eqref{eq:Rho0}, respectively, are a solution to the problem
\begin{align}
\tag{\ref{eq:DefSupLambda}}
\overline{\Lambda}_{\Theta} (\tilde{q},\tilde{v}) \triangleq \mathop{\sup}_{ \begin{array}{c}
\scriptstyle{q \sim \tilde{q}} \\ 
\scriptstyle{v \sim \tilde{v}} \end{array}}
\Lambda_{\Theta}(q,v).
\end{align}

2. The optimal value can be computed as
\begin{align}
\overline{\Lambda}_{\Theta} (\tilde{q},\tilde{v}) \triangleq & \sum_{j}{ \Big[ (|\Theta_j|-\mathsf{q}_j) \log{P\left(q=0|\ell^0(\mathsf{q}_j,\mathsf{V}^0_j)\right)}} \ + \nonumber \\
& \ \mathsf{q}_j \log{P\left(q=1|\ell^1(\mathsf{q}_j,\mathsf{V}^1_j)\right) \Big]},
\tag{\ref{eq:SolutionBigLambda}}
\end{align}
where
\begin{align}
\tag{\ref{eq:DefEll0}}
\ell^0(\mathsf{q}_j,\mathsf{V}^0_j) & \triangleq \sum_{i=1}^{N_r}{\log{\frac{r_i}{\rho^0_{j,i}(\mathsf{q}_j,\mathsf{v}^0_{j,i})}} },\ \text{and} \\
\tag{\ref{eq:DefEll1}}
\ell^1(\mathsf{q}_j,\mathsf{V}^1_j) & \triangleq \sum_{i=1}^{N_r}{\log{\frac{\rho^1_{j,i}(\mathsf{q}_j,\mathsf{v}^1_{j,i})}{r_{i-1}}} }. 
\end{align}

\begin{proof}
\hspace{-4pt}: 
Since the solution at each pixel $\Theta_j$ and its corresponding voxels $\Phi_{j,i}$ is independent of the solution at other pixels and their voxels, we focus without ambiguity in this proof on a general pixel $\Theta$ (\ie, $\Pi(\Theta) = \{ \Theta \}$) and its voxels $\{ \Phi_i \}$, dropping the pixel subscript $j$.

1) To prove that the continuous shapes $q^*$ and $v^*$ that maximize \eqref{eq:DefBigLambda} have the form depicted in Fig. \ref{fig:BoundProjection}, we prove that: (1a) $\Phi^1_i$ is completely filled ``before'' $\Phi^0_i$ starts to get filled; (1b) the mass in $\Phi^1_i$ is located on the inner side of $\Phi^1_i$; and (1c) the mass in $\Phi^0_i$ is located on the outer side of $\Phi^0_i$. Formally we have to prove the following points ($Cmp(\Phi)$, $Int(\Phi)$ and $Bnd(\Phi)$ denote, respectively, the \emph{complement}, \emph{interior} and \emph{boundary} of the set $\Phi$, as defined in \cite{Kah95}):

(1a) If there exists $\vec{X}_0 \in \left[v^* \cap Int(\Phi^0_i)\right]$, then $|v^* \cap \linebreak Int(\Phi^1_i)|=|\Phi^1_i|$.

(1b) The set $\varphi^1_i \triangleq \Theta^1 \times [r_{i-1},\rho^1_i(\mathsf{q},\tilde{v}(\Phi_i)))$ satisfies $\left|v^* \cap \varphi^1_i\right|=|\varphi^1_i|$ and $\left|v^* \cap (\Phi^1_i \setminus \varphi^1_i)\right|=0$.

(1c) The set $\varphi^0_i \triangleq \Theta^1 \times [\rho^0_i(\mathsf{q},\tilde{v}(\Phi_i)),r_i)$ satisfies $\left|v^* \cap \varphi^0_i\right|=|\varphi^0_i|$ and $\left|v^* \cap (\Phi^0_i \setminus \varphi^0_i)\right|=0$.

\emph{Proof of 1a.} By contradiction. Suppose that $q^*$ and $v^*$ maximize \eqref{eq:DefBigLambda}, that there exists $\vec{X}_0 \in \left[v^* \cap Int(\Phi^0_i)\right]$, and that $\left|v^* \cap Int(\Phi^1_i)\right|<|\Phi^1_i|$ (Fig. \ref{fig:SetupLemaProjectionTerm}a). 

\begin{figure}
\vspace{5pt}
\begin{center}
\includegraphics[width=0.9\columnwidth]{SetupLemaProjectionTerm.pdf}
\end{center}
\caption{(a) Setup for the proof of Lemma \ref{lem:UBProjectionTerm}-1a. (b) The continuous shape $v'$ constructed from $v^*$. See text for details.}
\vspace{-5pt}
\label{fig:SetupLemaProjectionTerm}
\end{figure}

Since the set $[v^* \cap Int(\Phi^0_i)]$ is open (because it is the intersection of two open sets), there exists $\varepsilon_0>0$ such that the open ball $\mathcal{B}(\vec{X}_0,\varepsilon_0)$ satisfies
\begin{equation}
\mathcal{B}(\vec{X}_0,\varepsilon_0) \subset \left[v^* \cap Int(\Phi^0_i)\right].
\end{equation}

Likewise, the set $\left[Int\left(Cmp(v^*)\right) \cap Int(\Phi^1_i)\right]$ is also open, and hence for a point $\vec{X}_1$ belonging to this set, there exist $\varepsilon_1>0$ such that 
\begin{equation}
\mathcal{B}(\vec{X}_1,\varepsilon_1) \subset [Int\left(Cmp(v^*)\right) \cap Int(\Phi^1_i)].
\end{equation}
That such a point $\vec{X}_1$ can be chosen is assured by the fact that $\left|Int\left(Cmp(v^*)\right) \cap Int(\Phi^1_i)\right| = |Cmp(v^*) \cap \linebreak Int(\Phi^1_i)| = |\Phi^1_i| - |v^* \cap Int(\Phi^1_i)| >0$ (since $v^*$ is a continuous shape and thus, according to Definition \ref{def:ContinuousShape}, it holds that $\left|Bnd(v^*)\right|=0$). 

Now let us define $\varepsilon = \min{ \{\varepsilon_0,\varepsilon_1\}}$ and consider the continuous shape $v'$ defined as (Fig. \ref{fig:SetupLemaProjectionTerm}b)
\begin{align}
v'(\vec{X}) \triangleq 
\left\{ \begin{array}{cl}
0, & \quad \text{if} \ \vec{X} \in \mathcal{B}[\vec{X}_0, \varepsilon], \\ 
1, & \quad \text{if} \ \vec{X} \in \mathcal{B}(\vec{X}_1, \varepsilon), \\ 
v^*(\vec{X}), & \quad \text{otherwise}. 
\end{array} \right.
\end{align}
It can be verified that $v' \sim \tilde{v}$ and that $\Lambda(q,v') > \Lambda(q,v^*)$, contradicting our assumption, and proving 1a. The remaining points (1b-c) are proven analogously. \qed

\emph{Proof of 2)} Follows simply by substituting the shapes $q^*$ and $v^*$ defined before into \eqref{eq:DefBigLambda}. \qed
\end{proof}
\end{lemma}

% Efficient Computation of Gamma.
\subsection{Efficient solution for $\Gamma_j(\mathsf{q}_j)$ defined in \eqref{eq:BigGamma}}
\label{sec:ComputationGamma}
In this section we show how to efficiently compute the function $\Gamma_j(\mathsf{q}_j)$ defined in \eqref{eq:BigGamma}. Since the solution at each pixel $\Theta_j$ is independent of the solution at other pixels, we focus without ambiguity on a general pixel $\Theta$ dropping the subscript $j$. We start by rewriting the function $\gamma (\mathsf{q}, \mathsf{V}^0, \mathsf{V}^1)$ defined in \eqref{eq:SmallGamma} as
\begin{align}
\gamma(\mathsf{q}, \mathsf{V}^0, \mathsf{V}^1) = \gamma^1(\mathsf{q}, \mathsf{V}^1) + \sum_{i=1}^{N_r}{\gamma^0_i(\mathsf{q}, \mathsf{v}^1_i, \mathsf{v}^0_i)},
\end{align}
where 
\begin{align}
\gamma^1(\mathsf{q}, \mathsf{V}^1) & \triangleq \mathsf{q} \log{\left(1-e^{\alpha \ell^1(\mathsf{q}, \mathsf{V}^1)}\right)} + \nonumber \\
& \quad \quad \frac{\lambda}{|J(T)|} \sum_{i=1}^{N_r}{\int^{|\Phi_i|}_{|\Phi_i|-\mathsf{v}^1_i}{\overline{D^{-1}_{H,\Phi_i}}(a)\ da}},
\end{align}
and
\begin{align}
\gamma^0_i(\mathsf{q}, \mathsf{v}^1_i, \mathsf{v}^0_i) &\triangleq \alpha (|\Theta|-\mathsf{q}) \log{\left(\frac{r_i}{\rho^0_i(\mathsf{q}, \mathsf{v}^0_i)}\right)} + \nonumber \\
& \quad \quad \frac{\lambda}{|J(T)|} \int^{|\Phi_i|-\mathsf{v}^1_i}_{|\Phi_i| - \mathsf{v}^0_i - \mathsf{v}^1_i}{\overline{D^{-1}_{H,\Phi_i}}(a)\ da}.
\end{align}

Using these definitions, and because $\gamma^1$ does not depend on $\mathsf{V}^0$, $\Gamma(\mathsf{q})$ can be written as
\begin{align}
\Gamma(\mathsf{q}) & = \Gamma^1(\mathsf{q}) + \sum_{i=1}^{N_r}{\Gamma^0_i(\mathsf{q}, \mathsf{v}^1_i)}, \ \text{where} \\
\label{eq:Gamma1}
\Gamma^1(\mathsf{q}) & \triangleq
 \left\{ \begin{array}{l}
\mathop{\sup}_{\mathsf{V}^1} \gamma^1(\mathsf{q}, \mathsf{V}^1), \\ 
s.t. \ 0 \le \mathsf{v}^1_i \le |\Phi^1_i| \quad (1 \le i \le N_r), 
\end{array} \right. \\
\label{eq:Gamma0}
\Gamma^0_i(\mathsf{q}, \mathsf{v}^1_i) & \triangleq 
\left\{ \begin{array}{l}
\mathop{\sup}_{\mathsf{v}^0_i} \gamma^0_i(\mathsf{q}, \mathsf{v}^1_i, \mathsf{v}^0_i), \\ 
s.t. \ 0 \le \mathsf{v}^0_i \le |\Phi^0_i|,
\end{array} \right.
\end{align}
and $\mathsf{v}^1_i$ in \eqref{eq:Gamma0} is the solution to \eqref{eq:Gamma1}. Now we need to show how to compute \eqref{eq:Gamma1} and \eqref{eq:Gamma0}.

The problem in \eqref{eq:Gamma0} can be solved analytically. Towards this end we compute ${\partial \gamma^0_i}/{\partial \rho^0_i}$ and set it to zero,
\begin{align}
\frac{\partial \gamma^0_i}{\partial \rho^0_i} & = -\frac{\alpha (|\Theta|- \mathsf{q})}{\rho^0_i} +  \nonumber \\  & \quad \quad \frac{\lambda}{|J(T)|} \overline{D^{-1}_{H,\Phi_i}}(|\Phi_i| - \mathsf{v}^1_i - \mathsf{v}^0_i) \frac{\partial \mathsf{v}^0_i}{\partial \rho^0_i} = \nonumber \\
& =-(|\Theta| - \mathsf{q}) \Big[\frac{\alpha}{\rho^0_i} + \nonumber \\
& \quad \quad \frac{\lambda}{|J(T)|} \overline{D^{-1}_{H,\Phi_i}}(|\Phi_i| - \mathsf{v}^1_i - \mathsf{v}^0_i){\rho^0_i}^2\Big] = 0.
\end{align}
This equation is satisfied when
\begin{align}
\rho^0_i = \sqrt[3]{\frac{-\alpha |J(T)|}{\lambda \overline{D^{-1}_{H,\Phi_i}}(|\Phi_i| - \mathsf{v}^1_i - \mathsf{v}^0_i)}}.
\end{align}

The problem in \eqref{eq:Gamma1}, on the other hand, is solved by a procedure similar to coordinate descent, noting that
\begin{align}
 \frac{\partial \gamma^1}{\partial \rho^1_i} & = \frac{-\alpha \mathsf{q} e^{\alpha \ell^1}}{1 - e^{\alpha \ell^1}} \frac{\partial \ell^1}{\partial \rho^1_i} + \frac{\lambda}{|J(T)|} \overline{D^{-1}_{H,\Phi_i}}(|\Phi_i| - \mathsf{v}^1_i) \frac{\partial \mathsf{v}^1_i}{\partial \rho^1_i} = \nonumber \\
& \frac{-\alpha \mathsf{q} e^{\alpha \ell^1}}{(1 - e^{\alpha \ell^1}) \rho^1_i} + \frac{\lambda}{|J(T)|} \mathsf{q} {\rho^1_i}^2 \overline{D^{-1}_{H,\Phi_i}} (|\Phi_i| - \mathsf{v}^1_i).
\end{align}
We refer the reader to the program code (that can be obtained from the authors by request) for further details.


==> TheoryOfShapes.tex <==
\section{Supplementary material: A theory of shapes}
\label{sec:TheoryOfShapes}

As mentioned before, SC algorithms have two parts: a FoAM and a BM. The FoAM was already mentioned in Section \ref{sec:SCAlgorithms} and described in detail in \cite[Section 5]{Rot10}. While the same FoAM can be used to solve many different problems, each BM is specific to a particular problem. In order to define the BM for the problem described in Section \ref{sec:LikelihoodDefinition}, in this section we introduce a mathematical framework that will allow us to compute the bounds.

To derive formulas to bound the evidence $L(H)$ of a hypothesis $H$ (the goal of the BM) for our specific problem of interest, we introduce in this section a framework to represent shapes and to compute bounds for their log-probability (in Section \ref{sec:EvidenceDefinition} we will show that this log-probability is closely related to the evidence). Three different shape representations will be introduced (Fig. \ref{fig:ShapeRepresentations}). Continuous shapes are the shapes that we would observe if our cameras (or 3D scanners) had ``infinite resolution.'' In that case it would be possible to compute the evidence $L(H)$ of a hypothesis with ``infinite precision" and therefore always select the (single) hypothesis whose evidence is maximum (except in concocted examples which have very low probability of occurring in practice). However, since real cameras and scanners have finite resolution, we introduce two other shape representations that are especially suited for this case: \emph{discrete} and \emph{semidiscrete} shape representations. Discrete shapes will allow us to compute a lower bound $\underline{L}(H)$ for the evidence of a hypothesis $H$. Semidiscrete shapes, on the other hand, will allow us to compute an upper bound $\overline{L}(H)$ for the evidence of a hypothesis $H$. Discrete and semidiscrete shapes are defined on partitions of the input image (i.e., non-overlapping regions that completely cover the image, see Fig. \ref{fig:Partitions}). Finer partitions result in tighter bounds, more computation, and the possibility of distinguishing more similar hypotheses. Coarser partitions on the other hand, result in looser bounds, less computation and more hypotheses that are indistinguishable (in the partition).

Previously we have assumed that the image domain, $\Omega \subset \mathbb{Z}^2$, consisted on discrete pixels arranged in a 2D grid. For reasons that will soon become clear, however, we assume from now on that the image domain $\Omega \subset \mathbb{R}^2$ is continuous. Thus, to discretize this continuouos domain we rely on ``partitions," defined next.

\begin{figure}
\vspace{-5pt}
\includegraphics[width=\columnwidth]{Figures/Partitions.pdf}
\caption{The set $\Omega$ and three possible partitions of it. Each square represents a partition element. $\Pi^2$ is finer than $\Pi^1$ ($\Pi^2 \le \Pi^1$). $\Pi^3$ is not comparable with neither $\Pi^1$ nor with $\Pi^2$.}
\vspace{-5pt}
\label{fig:Partitions}
\end{figure}

\begin{definition}[Partitions]
\label{def:Partitions}
Given a set $\Omega \subset {\mathbb R}^d$, a \emph{partition} $\Pi(\Omega)=\{{\Omega}_1,\dots,{\Omega}_n\}$ with ${\Omega}_i\ne \emptyset$, is a disjoint cover of the set $\Omega$ (Fig. \ref{fig:Partitions}). Formally, $\Pi(\Omega)$ satisfies
\begin{equation}
\bigcup^n_{i=1}{\Omega_i}=\Omega, \ \ \text{and} \  \ \Omega_i \cap \Omega_j=\emptyset \ \ \forall i\ne j. 
\label{eq:PartitionsConditions}
\end{equation}

A partition $\Pi(\Omega)=\{\Omega_1,\dots,\Omega_n\}$ is said to be \emph{uniform} if all the elements in the partition have the same measure $\left|\Omega_i\right|=\frac{\left|\Omega \right|}{n}$ for $i=1, \dots, n$. (Throughout this article we use the notation $\left|\Omega \right|$ to refer to, depending on the context, the measure or the cardinality of a set $\Omega$.) This measure is referred to as the \emph{unit size} of the partition. For $d=2$ and $d=3$, we will refer to the elements of the partition (${\Omega }_i$) as \emph{pixels} and \emph{voxels}, respectively.

Given two partitions $\Pi^1(\Omega)$ and $\Pi^2(\Omega)$ of a set $\Omega \subset {\mathbb R}^d$, $\Pi^2$ is said to be finer than $\Pi^1$, and $\Pi^1$ is said to be coarser than $\Pi^2$, if every element of $\Pi^2$ is a subset of some element of $\Pi^1$ (Fig. \ref{fig:Partitions}). We denote this relationship as $\Pi^2 \le \Pi^1$. Note that two partitions are not always comparable, thus the binary relationship ``$\le$'' defines a partial order in the space of all partitions.
\end{definition}

\subsection{Discrete shapes}
\label{sec:DiscreteShapes}
\begin{definition}[Discrete shapes]
\label{def:DiscreteShape}
Given a partition $\Pi(\Omega)$ of the set $\Omega \subset {\mathbb R}^d$, the \emph{discrete shape} $\hat{S}$ (Fig. \ref{fig:ShapeRepresentations}b) is defined as the function $\hat{S}:\Pi(\Omega) \to \{0,1\}$.
\end{definition}

\begin{figure}
\includegraphics[width=\columnwidth]{Figures/ShapeRepresentations.pdf}
\caption{The three different shape representations used in this article: the continuous shape $S$ (a), the discrete shape $\hat{S}$ (b), and the semidiscrete shape $\tilde{S}$ (c). $\hat{S}$ and $\tilde{S}$ are two approximations of $S$ in a finite partition (indicated by the red lines). The gray levels in $\tilde{S}$ represents how much of an element is full. See text for details.}
\vspace{-15pt}
\label{fig:ShapeRepresentations}
\end{figure}

\begin{definition}[Log-probability of a discrete shape]
\label{def:LogPDiscreteShape}
Let $\hat{S}$ be a discrete shape in some partition $\Pi(\Omega)=\{\Omega_1,\dots,\Omega_n\}$, and let $\hat{B}=\{\hat{B}_1,\dots,\hat{B}_n\}$ be a family of independent Bernoulli random variables referred to as a discrete Bernoulli field (BF). Let $\hat{B}$ be characterized by the success rates $p_{\hat{B}}(i) \triangleq P({\hat{B}}_i=1) \in (\varepsilon,1-\varepsilon)$ for $i=1, \dots, n$, and $0<\varepsilon \ll 1$. To avoid the problems derived from assuming complete certainty, i.e. success rates of 0 or 1, following Cromwell's rule \cite{Lin85}, we will only consider success rates in the open interval $(\varepsilon,1-\varepsilon)$.

The \emph{log-probability of a discrete shape} is defined as
\begin{align}
\log {P(\hat{B}=\hat{S})} & \triangleq \sum_{i=1}^n{\log P\left(\hat{B}_i=\hat{S}(\Omega_i)\right)} \nonumber \\
& = \sum_{i=1}^n{\bigg[\left(1 - \hat{S}(\Omega_i)\right) \log{P\left(\hat{B}_i=0 \right)} + }\nonumber \\ 
& \qquad \qquad \hat{S}(\Omega_i) \log{P\left(\hat{B}_i=1 \right)} \bigg] \nonumber \\
& = Z_{\hat{B}} + \sum_{i=1}^n{\hat{S}(\Omega_i)\delta_{\hat{B}}(i)},
\label{eq:LogPDiscreteShape}
\end{align}
where $Z_{\hat{B}} \triangleq \sum_{i=1}^n{\log \left(1-p_{\hat{B}}(i)\right)}$ is a constant and $\delta _{\hat{B}}(i) \triangleq {\log \left({p_{\hat{B}}(i)} / {\left(1-p_{\hat{B}}(i)\right)}\right)}$ is the logit function of $p_{\hat{B}}(i)$.
\end{definition}

The discrete BFs used in this work arise from two sources: background subtraction and shape priors. To compute a discrete BF ${\hat{B}}_f$ using the \emph{Background Subtraction} technique \cite{Mit04}, recall the probability densities $p_{\Omega_i}\left(f(\Omega_i) | q(\Omega_i)=0\right)$ and $p_{\Omega_i}\left(f(\Omega_i) | q(\Omega_i)=1\right)$ defined in Section \ref{sec:ProblemDefinition} to model the probability of observing a feature $f(\Omega_i)$ at a given pixel $\Omega_i$, depending on the pixel's state $q(\Omega_i)$. The success rates of the discrete BF $\hat{B}_f$ are thus defined as 
\begin{equation}
p_{\hat{B}_f}(i) \triangleq \frac{p_{\Omega_i}(f(\Omega_i) | q(\Omega_i) = 1)} {p_{\Omega_i}(f(\Omega_i) | q(\Omega_i)=0) + p_{\Omega_i}(f(\Omega_i) | q(\Omega_i)=1)}.
\label{eq:BFBackgrounSubtraction}
\end{equation}

To compute a discrete BF $\hat{B}_s$ associated with a \emph{discrete shape prior}, we can estimate the success rates $p_{\hat{B}_s}(i)$ of $\hat{B}_s$ from a collection of $N$ discrete shapes, $\hat{\Sigma}=\left\{\hat{S}_1,\dots,\hat{S}_N\right\}$, assumed to be aligned in the set $\Omega$. These discrete shapes can be acquired by different means, e.g., using a 2D or 3D scanner, for $d=2$ or $d=3$, respectively. The success rate $p_{\hat{B}_s}(i)$ of a particular Bernoulli variable $\hat{B}_i$ ($i=1, \dots, n$) is thus estimated from $\left\{\hat{S}_1(\Omega_i),\dots,\right.$ $\left. \hat{S}_N(\Omega_i)\right\}$ using the standard formula for the estimation of Bernoulli distributions \cite{Kay93},
\begin{equation}
p_{\hat{B}_s}(i)=\frac{1}{N}\sum^N_{j=1}{\hat{S}_j(\Omega_i)}.
\label{eq:BFFromTrainingSet}
\end{equation}

Discrete shapes, as in Definition \ref{def:DiscreteShape}, have two limitations that must be addressed to enable subsequent developments. First, the log-probability in \eqref{eq:LogPDiscreteShape} depends (implicitly) on the unit size of the partition (which is related to the image resolution), preventing the comparison of log-probabilities of images acquired at different resolutions (this will be further explained after Definition \ref{def:LogPContinuousShape}). Second, it was assumed in \eqref{eq:LogPDiscreteShape} that the Bernoulli variables $\hat{B}_i$ and the pixels $\Omega_i$ were perfectly aligned. However, this assumption might be violated if a transformation (e.g., a rotation) is applied to the shape. To overcome these limitations, and also to facilitate the proofs that will follow, we introduce next the second shape representation, that of a continuous shape.

\subsection{Continuous shapes}
\label{sec:ContinuousShapes}
\begin{definition}[Continuous shapes]
\label{def:ContinuousShape}
Given a set $\Omega \subset {\mathbb R}^d$, we define a \emph{continuous shape} $S$ to be a function $S:\Omega \to \{0,1\}$ (Fig. \ref{fig:ShapeRepresentations}a). We will often abuse notation and refer to the set $S=\left\{\vec{x} \in \Omega:S(\vec{x})=1\right\}$ also as the shape. To avoid pathological cases, we will require the set $S$ to satisfy two regularity conditions: 1) to be open (in the usual topology in ${\mathbb R}^d$ \cite{Kah95}) and 2) to have a boundary (as defined in \cite{Kah95}) of measure zero.
\end{definition}

Given a discrete shape $\hat{S}$ defined on a partition $\Pi(\Omega)=\left\{\Omega_1,\dots,\Omega_n\right\}$, the continuous shape $S(\vec{x}) \triangleq \hat{S}(\Omega_i) \ \forall \vec{x} \in \Omega_i$, is referred to as the continuous shape \emph{produced} by the discrete shape $\hat{S}$, and is denoted as $S \sim \hat{S}$ or $\hat{S} \sim S$. Intuitively, $S$ extends $\hat{S}$ from every element of $\Pi(\Omega)$ to every point $\vec{x} \in \Omega$.

We would like now to extend the definition of the log-probability of a discrete shape (in Definition \ref{def:LogPDiscreteShape}) to include continuous shapes. Toward this end we first introduce continuous BFs, which play in the continuous case the role that discrete BFs play in the discrete case.

\begin{definition}[Continuous Bernoulli Fields]
\label{def:ContinuousBF}
Given a set $\Omega \subset {\mathbb R}^d$, a \emph{continuous Bernoulli field} (or simply a BF) is the construction that associates a Bernoulli random variable $B_{\vec{x}}$ to every point $\vec{x} \in \Omega$. The \emph{success rate} for each variable in the field is given by the function $p_B(\vec{x}) \triangleq P(B_{\vec{x}}=1)$. The corresponding \emph{logit function} $\delta_B(\vec{x}) \triangleq {\log \left(\frac{p_B(\vec{x})} {1-p_B(\vec{x})}\right)}$ and \emph{constant term} $Z_B \triangleq \int_\Omega{{\log \left(1-p_B(\vec{x})\right) }d\vec{x}}$ are as in Definition \ref{def:LogPDiscreteShape}.
\end{definition}

We will only consider in this work functions $p_B(\vec{x})$ such that $\left|Z_B\right|<\infty$ and $\delta_B(\vec{x})$ is a measurable function \cite{Wil78}. Furthermore, since $\varepsilon<p_B(\vec{x})<1-\varepsilon \ \forall \vec{x} \in \Omega$, $\delta_B(\vec{x}) \in (-\delta_{max},\delta_{max}) \ \forall \vec{x} \in \Omega$, with $\delta_{max} \triangleq {\log  \left(\frac{1-\varepsilon }{\varepsilon}\right)}$. Note that a BF is \emph{not} associated to a \emph{continuous} probability density on $\Omega$ (e.g., it almost never holds that $\int_{\Omega }{p_B(\vec{x})\ d\vec{x}}=1$), but rather to a collection of \emph{discrete} probability distributions, one for each point in $\Omega$ (thus, it always holds that $P\left(B_{\vec{x}}=0\right)+P\left(B_{\vec{x}}=1\right)=1\ \forall \vec{x}\in \Omega$). 

Due to the finite resolution of cameras and scanners, continuous BFs cannot be directly obtained as discrete BFs were obtained in Definition \ref{def:LogPDiscreteShape}. In contrast, continuous BFs are obtained indirectly from discrete BFs (which are possibly obtained by one of the methods described in Definition \ref{def:LogPDiscreteShape}). Let $\hat{B}$ be a discrete BF defined on a partition $\Pi(\Omega)=\left\{\Omega_1,\dots,\Omega _n\right\}$. Then, for each partition element $\Omega_i$, and for each point $\vec{x}\in \Omega_i$, the success rate of the Bernoulli variable $B_{\vec{x}}$ is defined as $p_B(\vec{x}) \triangleq p_{\hat{B}}(i)$. The BF $B$ produced in this fashion will be referred to as the BF \emph{produced} by the discrete BF $\hat{B}$. Intuitively, $p_B$ extends $p_{\hat{B}}$ from every element of $\Pi(\Omega)$ to every point $\vec{x} \in \Omega$. Note that this definition is analogous to the definition of a continuous shape produced from a discrete shape in Definition \ref{def:ContinuousShape}.

Let $\Omega' \subset {\mathbb R}^d$ be a set referred to as the \emph{canonical set}, let $\Omega \subset {\mathbb R}^d$ be a second set referred to as the \emph{world set}, and let $T:\Omega' \to \Omega$ be a bijective transformation between these sets. Given a BF $B$ in $\Omega'$ with success rates $p_B(\vec{x})$, the transformed BF $B_T$ in $\Omega$ is defined as $B_T \triangleq B \circ T^{-1}$ with success rates $p_{B_T}(\vec{x}) \triangleq p_B\left(T^{-1}\vec{x}\right)$.

\begin{definition}[Log-probability of a continuous sha\-pe]
\label{def:LogPContinuousShape}
Let $B$ be a BF in $\Omega$ with success rates given by the function $p_B(\vec{x})$, let $S$ be a continuous shape also in $\Omega$, and let $u_o>0$ be a scalar called the \emph{equivalent unit size}. We define the \emph{log-probability that a shape $S$ is produced by a BF $B$}, by extension of the log-probability of discrete shapes in \eqref{eq:LogPDiscreteShape}, as
\begin{equation}
\log P(B=S) \triangleq \frac{1}{u_o} \left[Z_B + \int_{\Omega}{S(\vec{x}) \delta_B(\vec{x})\ d\vec{x}}\right],
\label{eq:LogPContinuousShape}
\end{equation}

\noindent where $Z_B$ and ${\delta }_B$ are respectively the constant term and the logit function of $B$.
\end{definition}

Several things are worth noting in this definition. First, note that if there is a uniform partition $\Pi(\Omega)=\left\{\Omega_1,\dots,\Omega_n\right\}$ with $\left|\Omega_i\right|=u_o\ \forall i$, and if the continuous shape $S$ and the BF $B$ are respectively produced by the discrete shape $\hat{S}$ and the discrete Bernoulli field $\hat{B}$ defined on $\Pi(\Omega)$, then $\log P(B=S)= \log P\left(\hat{B}=\hat{S}\right)$. For this reason we said that the definition in \eqref{eq:LogPContinuousShape} extends the definition in \eqref{eq:LogPDiscreteShape}. However, keep in mind that in the case of a continuous shape \eqref{eq:LogPContinuousShape} \emph{is not a log-probability in the traditional sense}, but rather it extends the definition to cases in which $S(\vec{x})$ is not produced from a discrete shape and $\delta_B(\vec{x})$ is not piecewise constant in a partition of $\Omega$.

Second, note that while \eqref{eq:LogPContinuousShape} provides the ``log-pro\-ba\-bi\-lity" density that a given continuous shape is produced by a BF, sampling from a BF is not guaranteed to produce a continuous shape (because the resulting set might not satisfy the regularity conditions in Definition \ref{def:ContinuousShape}). Nevertheless, this is not an obstacle since in this work we are only interested in computing log-probabilities of continuous shapes that are given, not on sampling from BFs.

Third, note in \eqref{eq:LogPContinuousShape} that the log-probability of a continuous shape is the product of two factors: 1) the inverse of the unit size, which only depends on the partition (but not on the shape); and 2) a term (in brackets) that does not depend on the partition. In the case of continuous shapes, $u_o$ in the first factor is not the unit size of the partition (there is no partition defined in this case) but rather a scalar defining the unit size of an \emph{equivalent partition} in which the range of log-probability values obtained would be comparable. The second factor is the sum of a constant term that only depends on the BF $B$, and a second term that also depends on the continuous shape $S$.

Fourth, the continuous shape representation in Definition \ref{def:ContinuousShape} overcomes the limitations of the discrete representation pointed out above. More specifically, by considering continuous shapes, \eqref{eq:LogPContinuousShape} can be computed even if a discrete shape and a discrete BF are defined on partitions that are not aligned, allowing us greater freedom in the choice on the transformations ($T$) that can be applied to the BF. Furthermore, the role of the partition is ``decoupled'' from the role of the BF and the shape, allowing us to compute \eqref{eq:LogPContinuousShape} independently of the resolution of the partitions. 

\subsection{Semi-discrete shapes}
\label{sec:SemiDiscreteShapes}
As mentioned at the beginning of this section, discrete shapes will be used to obtain a lower bound for the log-probability of a continuous shape. Unfortunately, upper bounds for the log-probability derived using discrete shapes are not very tight. For this reason, to obtain upper bounds for this log-probability, we need to introduce the third shape representation, that of semidiscrete shapes.

\begin{definition}[Semidiscrete shapes]
\label{def:SemidiscreteShape}
Given a partition $\Pi(\Omega)=\left\{\Omega_1,\dots,\Omega_n\right\}$ of the set $\Omega \subset {\mathbb R}^d$, the \emph{semidiscrete shape} $\tilde{S}$ is defined as the function $\tilde{S}:\Pi(\Omega) \to [0,|\Omega|]$, that associates to each element $\Omega_i$ in the partition a real number in the interval $[0,\left|\Omega _i\right|]$, i.e., $\tilde{S}(\Omega_i) \in [0,\left|\Omega_i\right|]$ (Fig. \ref{fig:ShapeRepresentations}c).
\end{definition}

Given a continuous shape $S$ in $\Omega$, we say that this shape \emph{produces} the semidiscrete shape $\tilde{S}$, denoted as $S \sim \tilde{S}$ or $\tilde{S} \sim S$, if $\tilde{S}(\Omega_i)=|S \cap \Omega_i|$ for $i=1, \dots, n$. An intuition that will be useful later to understand the derivation of the upper bounds is that a semidiscrete shape produced from a continuous shape ``remembers'' the measure of the continuous shape inside each element of the partition, but ``forgets" where exactly the shape is located inside the element.

Given two continuous shapes in $\Omega$, $S_1$ and $S_2$, that produce the the same semidiscrete shape $\tilde{S}$ in the partition $\Pi(\Omega)$, we say the these continuous shapes are related (denoted as $S_1 \sim S_2$). The nature of this relationship is explored in the next proposition.

\begin{proposition}[Equivalent classes of continuous shapes]
\label{prop:EquivalentClassesOfShapes}
The relationship ``$\sim$'' defined above is an equivalence relation.
\begin{proof}
The proof of this proposition is trivial from Definition \ref{def:SemidiscreteShape}. \qed
\end{proof}
\end{proposition}
We will say that these continuous shapes are equivalent in the partition $\Pi(\Omega)$, and by extension, we will also say that they are equivalent to $\tilde{S}$ (i.e., $S_i \sim \tilde{S}$).

\begin{proposition}[Relationships between shape representations]
\label{prop:RelationshipsBetweenShapes}
Let $\Pi(\Omega)=\left\{\Omega_1,\dots,\Omega_n\right\}$ be an arbitrary partition of a set $\Omega$, and let $\widehat{\mathbb S}(\Pi)$ and $\widetilde{\mathbb S}(\Pi)$ be the sets of all discrete and semidiscrete shapes, respectively, defined on $\Pi(\Omega)$. Let ${\mathbb S}$ be the set of all continuous shapes in $\Omega $. Then,
\begin{align}
\label{eq:DiscreteShapesInContinuousShapes}
\left\{S:S \sim \hat{S}, \hat{S} \in \widehat{\mathbb S}(\Pi)\right\} & \subset \mathbb{S},\ \  \text{and}, \\
\label{eq:SemiDiscreteShapesEqualContinuousShapes}
\left\{S:S \sim \tilde{S},\tilde{S} \in \widetilde{\mathbb S}(\Pi)\right\} & = \mathbb{S}.
\end{align}

\begin{proof}
The proof of this proposition is trivial from definitions \ref{def:DiscreteShape}, \ref{def:ContinuousShape}, and \ref{def:SemidiscreteShape}. \qed
\end{proof}
\end{proposition}

\subsection{LCDFs and summaries}
\label{sec:LCDFSandSummaries}
So far we have introduced three different shape representations and established relationships among them. In this section we introduce the concepts of logit cumulative distribution functions (LCDFs) and summaries. These concepts will be necessary to use discrete and semidiscrete shapes to bound the log-probability of continuous shapes, and hence, to bound the evidence.

Intuitively, a LCDF ``condenses'' the ``information'' of a BF in a partition element into a monotonous function. A summary then further ``condenses'' this ``information'' into a single vector of fixed length. Importantly, the summary of a BF in a partition element can be used to bound the evidence $L(H)$ and can be computed in constant time, regardless of the number of pixels in the element. 

After formally defining LCDFs and summaries below, we will prove in this Section some of the properties that will be needed in Section \ref{sec:BoundingMechanism} to compute lower and upper bounds for $L(H)$. In the remainder of this section, unless stated otherwise, all partitions, shapes and BFs are defined on a set $\Omega \subset {\mathbb R}^d$.

\begin{definition}[Logit cumulative distribution function]
\label{def:LCDFs}
Given the logit function $\delta_B$ of a BF $B$ and a partition $\Pi$, the \emph{logit cumulative distribution function} (or LCDF) of the BF $B$ in $\Pi$ is the collection of functions $D_B={\left\{D_{B,\omega}\right\}}_{\omega \in \Pi}$, where each function $D_{B,\omega}:[-\delta_{max},\delta_{max}] \to \left[0,\left|\omega\right|\right]$ is defined as
\begin{equation}
\label{eq:LCDF_D}
D_{B,\omega}(\delta) \triangleq \left|\left\{\vec{x} \in \omega:\delta_B(\vec{x})<\delta \right\}\right| \ (\omega \in \Pi).
\end{equation}
\end{definition}

It must be noted that this definition is consistent, since from Definition \ref{def:ContinuousBF}, the logit function is measurable. The LCDF is named by analogy to the probability cumulative distribution function, but must not be confused with it. Informally, a LCDF ``condenses'' the information of the BF by ``remembering'' the values taken by the logit function inside each partition element, but ``forgetting'' where those values are inside the element. This relationship between BFs and their LCDFs is analogous to the relationship between continuous and semidiscrete shapes.

Equation \eqref{eq:LCDF_D} defines a non-decreasing and possibly discontinuous function. To see that this function is non-decreasing, note that the set $\chi_1 \triangleq \{\vec{x} \in \omega:\delta_B(\vec{x})<\delta_1 \}$ is included in the set $\chi_2 \triangleq \{\vec{x} \in \omega:\delta_B(\vec{x})<\delta_2 \}$ if $\delta_1 \le \delta_2$. Moreover, this function is not necessarily strictly increasing because it is possible to have $D_{B,\omega}(\delta_1)=D_{B,\omega}(\delta_2)$ with $\delta_1<\delta_2$ if the measure of the set $\{\vec{x} \in \omega: \delta_1 \le \delta_B(\vec{x}) < \delta_2  \}$ is zero. To see that the function defined in \eqref{eq:LCDF_D} can be discontinuous, note that this function will have a discontinuity whenever the function $\delta_B(\vec{x})$ is constant on a set of measure greater than zero.

Later in this section we will use the inverse of a LCDF, $D^{-1}_{B,\omega}(a)$. If $D_{B,\omega}(\delta)$ were strictly increasing and continuous, we could simply define $D^{-1}_{B,\omega}(a)$ as the unique real number $\delta \in \left[-\delta_{max},\delta_{max}\right]$ such that $D_{B,\omega}(\delta)=a$. For general LCDFs, however, this definition does not produce a value for every $a \in \left[0,\left|\omega\right|\right]$. Instead we use the following definition.

\begin{definition}[Inverse LCDF]
\label{def:InverseLCDF}
The \emph{inverse LCDF} $D^{-1}_{B,\omega}(a)$ is defined as (see Fig. \ref{fig:LCDFs})
\begin{equation}
\label{eq:InverseLCDF}
D^{-1}_{B,\omega}(a) \triangleq \inf \left\{\delta:D_{B,\omega}(\delta) \ge a\right\}.
\end{equation}
To avoid pathological cases, we will only consider in this work LCDFs whose inverse is continuous almost everywhere (note that this imposes an additional restriction on the logit function).
\end{definition}

\begin{figure}
\vspace{-5pt}
\includegraphics[width=\columnwidth]{Figures/LCDFs.pdf}
\vspace{-15pt}
\caption{Plot of the LCDF $a=D_{B,\omega}(\delta)$ (left) and its inverse $\delta=D^{-1}_{B,\omega}(a)$ (right). The shaded area under the curve on the right is the maximal value of the integral on the rhs of \eqref{eq:LemaPart1} for any BF $B \sim D_{B,\omega}$ (see Lemma \ref{lem:PropertiesLCDFsAndSummaries}).}
\vspace{-15pt}
\label{fig:LCDFs}
\end{figure}

\begin{definition}[X-axis crossing point]
\label{def:XCrossingPoint}
We define the \emph{x-axis crossing point}, $A_{B,\omega}$, as
\begin{equation}
\label{eq:XCrossingPoint}
A_{B,\omega} \triangleq \frac{D_{B,\omega}(0^-)+D_{B,\omega}(0^+)}{2}.
\end{equation}
\end{definition}
This quantity has the property that $D^{-1}_{B,\omega}(a) \ge 0$ if $a \ge A_{B,\omega}$, and $D^{-1}_{B,\omega}(a) \le 0$ if $a \le A_{B,\omega}$.

\begin{definition}[Summaries]
\label{def:Summaries}
Given a partition $\Pi$, a \emph{summary} of a LCDF $D_B={\left\{D_{B,\omega}\right\}}_{\omega \in \Pi}$ in the partition is a functional that assigns to each function $D_{B,\omega}$ ($\omega \in \Pi$) in the LCDF a vector $Y_{B,\omega} \in {\mathbb R}^{d_Y}$. The name ``summary'' is motivated by the fact that the ``infinite dimensional'' distribution is ``summarized'' by just $d_Y$ real numbers.

Two types of summaries are used in this article: \emph{m}-summaries and mean-summaries. Given $m>0$, an \emph{m-summary} assigns to each function $D_{B,\omega}$ in the LCDF the $(2m+1)$-dimensional vector $\tilde{Y}_{B,\omega} = \left[\tilde{Y}^{-m}_{B,\omega} \right. \dots$ ${\left. \tilde{Y}^m_{B,\omega}\right]}^T$ of equispaced samples of the LCDF, i.e.,
\begin{equation}
\label{eq:MSummary}
\tilde{Y}^j_{B,\omega} \triangleq D_{B,\omega}\left(\frac{j\delta_{max}}{m}\right) \ \ (j=-m,\dots ,m).
\end{equation}
Note that since the LCDF is known to be a non-decrea\-sing function, the information in the \emph{m}-summary can be used to bound the inverse LCDF (Fig. \ref{fig:BoundLCDFs}). Specifically, we know that $D^{-1}_{B,\omega}(a) \le \frac{\delta_{max}} {m} (j+1)$ for $a \in \left[\tilde{Y}^j_{B,\omega},\right.$ $\left. \tilde{Y}^{j+1}_{B,\omega}\right]$, which can be written as 
\begin{align}
D^{-1}_{B,\omega}(a) & \le \overline{D^{-1}_{Y_{B,\omega}}}(a) \nonumber \\
& \triangleq \frac{\delta_{max}}{m} J(a),\ \forall a \in \left[0,\left|\omega\right|\right],
\label{eq:DInverseUpper}
\end{align}
with
\begin{align}
J(a) & \triangleq \min \left\{j:\tilde{Y}^j_{B,\omega} \ge a\right\} \nonumber \\
& =\left|\left\{j:\tilde{Y}^j_{B,\omega}<a\right\}\right|-m.
\label{eq:J}
\end{align}
These bounds will be used in turn to compute an upper bound for $L(H)$.

\begin{figure}
\vspace{-10pt}
\begin{center}
\includegraphics[width=0.85\columnwidth]{Figures/BoundLCDFs.pdf}
\end{center}
\vspace{-10pt}
\caption{Lower (in orange) and upper (in green) bounds for the inverse LCDF $\delta=D_{B,\omega}^{-1}(a)$ (in black) computed from the \emph{m}-summaries with $m=2$. The $j$-th component of the summary, $\tilde{Y}_{B,\omega}^j$, is represented by a dotted vertical line at the horizontal position $a=\tilde{Y}_{B,\omega}^j$ (or where $D_{B,\omega}^{-1}(a)=\delta_j \triangleq j \delta_{max} / m$).}
\vspace{-15pt}
\label{fig:BoundLCDFs}
\end{figure}

The second type of summaries, referred to as mean-summaries, will be used to compute a lower bound of $L(H)$. The \emph{mean-summary} assigns to each function $D_{B,\omega}$ the scalar
\begin{equation}
\label{eq:MeanSummary}
\hat{Y}_{B,\omega} \triangleq \int_0^{|\omega|} {D^{-1}_{B,\omega}(a)\ da} = \int_{\omega}{\delta_B(\vec{x})\ d\vec{x}}.
\end{equation}
The last equality follows by setting $\tilde{S}(\omega)=|\omega|$ in \eqref{eq:LemaPart1} and is proved later in Lemma \ref{lem:PropertiesLCDFsAndSummaries}. Note that this equality provides the means to compute the mean-summary directly from the logit function, without having to compute the LCDF.
\end{definition}

\input ComputingSummaries

To derive formulas to bound $L(H)$, we need the following two results.

\begin{proposition}[Equivalent classes of BFs]
\label{prop:EquivalentClassesOfBFs}
Let $\Pi$ be a partition, let $B_1$ and $B_2$ be two BFs, and consider the following binary relations: 1) $B_1$ and $B_2$ are related (denoted as $B_1\sim_D B_2$) if they produce the same LCDF $D={\left\{D_{\omega}\right\}}_{\omega \in \Pi}$; and 2) $B_1$ and $B_2$ are related (denoted as $B_1\sim_Y B_2$) if they produce the same summary $Y={\left\{Y_{\omega}\right\}}_{\omega \in \Pi}$. Then, ``$\sim_D$" and ``$\sim_Y$" are equivalence relations.
\begin{proof}
Immediate from definitions \ref{def:LCDFs} and \ref{def:Summaries}.\qed
\end{proof}
\end{proposition}

In the first case ($\sim_D$) we will say that these BFs are \emph{equivalent} in the partition $\Pi$ \emph{with respect to distributions}. Abusing the notation, we will also say that they are equivalent to (or \emph{compatible with}) the LCDF (i.e., $B_i\sim D$). Similarly, in the second case ($\sim_Y$) we will say that these BFs are \emph{equivalent} in the partition $\Pi$ \emph{with respect to summaries}. Abusing the notation, we will also say that they are equivalent to (or \emph{compatible with}) the summary (i.e., $B_i\sim Y$). Note that if two BFs are equivalent with respect to a LCDF, they are also equivalent with respect to any summary of the LCDF. The reverse, however, is not necessarily true.

\begin{lemma}[Properties of LCDFs and \emph{m}-Su\-mma\-ries]
\label{lem:PropertiesLCDFsAndSummaries}
Let $\Pi$ be an arbitrary partition, and let $\tilde{S}$ and $D={\left\{D_{\omega}\right\}}_{\omega \in \Pi}$ be respectively a semidiscrete shape and a LCDF in this partition. Then:

1. Given a BF $B$ such that $B\sim D$, it holds that (Fig. \ref{fig:LCDFs})
\begin{equation}
\label{eq:LemaPart1}
\mathop{\sup}_{S\sim \tilde{S}} \int_{\Omega}{\delta_B(\vec{x})S(\vec{x})\ d\vec{x}} = 
\sum_{\omega \in \Pi}{\int^{\left|\omega\right|}_{\left|\omega\right|-\tilde{S}(\omega)} {D^{-1}_{\omega}(a)\ da}}.
\end{equation}

2. Similarly, given a continuous shape $S$, such that $S\sim \tilde{S}$, it holds that
\begin{equation}
\label{eq:LemaPart2}
\mathop{\sup}_{B\sim D} \int_{\Omega}{\delta_B(\vec{x})S(\vec{x})\ d\vec{x}} =
\sum_{\omega \in \Pi} {\int^{\left|\omega\right|}_{\left|\omega\right|-\tilde{S}(\omega)} {D^{-1}_{\omega}(a)\ da}}.
\end{equation}

3. Moreover, for any $\alpha \in \left[0, |\omega|\right]$, the integrals on the rhs of \eqref{eq:LemaPart1} and \eqref{eq:LemaPart2} can be bounded as
\begin{align}
\int^{\left|\omega\right|}_{\alpha}{D^{-1}_{\omega}(a)\ da} \le \frac{\delta_{max}}{m} \left[ 
\vphantom{\sum^{m-1}_{j=J(\alpha)}{\left(\tilde{Y}^{j+1}_{\omega}\right)(j+1)}}
J(\alpha)\left(\tilde{Y}^{J(\alpha)}_{\omega}-\alpha \right) + \right. \nonumber \\
\label{eq:LemaPart3}
\left. \sum^{m-1}_{j=J(\alpha)}{\left(\tilde{Y}^{j+1}_{\omega}-\tilde{Y}^j_{\omega}\right)(j+1)} \right],
\end{align}
where $J(\alpha)$ is as defined in \eqref{eq:J}.

4. The rhs of \eqref{eq:LemaPart1} and \eqref{eq:LemaPart2} are maximum when $\tilde{S}(\omega)=|\omega|-A_{\omega}$, thus
\begin{equation}
\label{eq:LemaPart4}
\mathop{\sup}_{\tilde{S}} \sum_{\omega \in \Pi} {\int^{|\omega|}_{|\omega|-\tilde{S}(\omega)}{D^{-1}_{\omega}(a)\ da}} = 
\sum_{\omega \in \Pi} {\int^{|\omega|}_{A_{\omega}}{D^{-1}_{\omega}(a)\ da}}.
\end{equation}

This lemma is proved in \cite{Rot10}.
\end{lemma}

This concludes the presentation of the general mathematical framework to compute and bound probabilities of shapes.

